A Systematic Review of Echo Chamber Research: Comparative Analysis of Conceptualizations, Operationalizations, and Varying Outcomes

This systematic review synthesizes research on echo chambers and filter bubbles to explore the reasons behind dissent regarding their existence, antecedents, and effects. It provides a taxonomy of conceptualizations and operationalizations, analyzing how measurement approaches and contextual factors influence outcomes. The review of 129 studies identifies variations in measurement approaches, as well as regional, political, cultural, and platform-specific biases, as key factors contributing to the lack of consensus. Studies based on homophily and computational social science methods often support the echo chamber hypothesis, while research on content exposure and broader media environments, such as surveys, tends to challenge it. Group behavior, cultural influences, instant messaging platforms, and short video platforms remain underexplored. The strong geographic focus on the United States further highlights the need for studies in multi-party systems and regions beyond the Global North. Future research should prioritize cross-platform studies, continuous algorithmic audits, and investigations into the causal links between polarization, fragmentation, and echo chambers to advance the field. This review also provides recommendations for using the EUs Digital Services Act to enhance research in this area and conduct studies outside the US in multi-party systems. By addressing these gaps, this review contributes to a more comprehensive understanding of echo chambers, their measurement, and their societal impacts.

==> Tables/Table_StructuralAnalysis.tex <==
\let\cline\cmidrule

\begin{small}
\begin{table}[]
    \centering
    \begin{tabular}{p{3cm}p{2cm}p{3.5cm}p{5cm}}
\rowcolor{black}
\multicolumn{4}{c}{\color{white} \textbf{CODEBOOK}} \\ \hline
\multicolumn{1}{c}{\textbf{Code}} &
\multicolumn{1}{c}{\textbf{Subcode}} &
\multicolumn{1}{c}{\textbf{Value Range}}&
\multicolumn{1}{c}{\textbf{Code Description}} \\ \hline 

\multirow{2}{3cm}
{FOCUS AND GRANULARITY: What are the foci of the publication and which factors / conceptualizations of echo chambers are used?} & Focus &EC hypothesis, News sharing and consumig, Recommender Systems and EC, "Cognitive states, personality traits, and EC", Opinion dynamics on social media, ''COVID-19, vaccines and EC``, Misinformation and EC, "Extremism, radicalization and EC", Elections and EC, Climate change and EC, Migitation of EC, Parliament discussions and EC& What is the primary focus of the publication regarding echo chamber research on social media?  \\ 
\cline{2-4} 

& Group & "Yes" / "No" &Does the publication analyze a specific group for echo chamber properties? \\
\cline{2-4}

& Platform &"Yes" / "No"&Does the publication explore echo chambers on specific social media platforms? \\
\cline{2-4}

& Cross-Platform & "Yes" / "No"&Does the publication examine echo chambers across multiple social media platforms? \\
\cline{2-4}

& Holistic & "Yes" / "No" &Does the publication take a holistic approach to studying echo chambers, considering various platforms and media simultaneously? \\

\hline

\multirow{2}{3cm}
{EC CONSTRUCT AND CONCEPTUALIZATION: Which factors and conceptualizations of echo chambers are used to analyze echo chambers?} & Well-defined conceptualization?& "Yes" / "No" & Is the definition of an echo chamber well-defined in the publication?\\
\cline{2-4}


&Homophily & "Yes" / "No" &Does the publication consider homophily as a conceptualization of echo chambers? \\ 
\cline{2-4} 

& Content Exposure & "Yes" / "No" &Does the publication conceptualize echo chambers through content exposure, i.e. which content is circulating in a network or group? \\
\cline{2-4}

& User Behaviour & "Yes" / "No" &Did the authors use specific user behavior like confirmation bias or selective exposure as a factor for defining an echo chamber?\\
\cline{2-4}

& Group Behaviour& "Yes" / "No" &Did the authors use a specific group behavior like discrediting of non-members of the group and active exclusion as a factor of echo chambers?  \\
\cline{2-4}

& Recommender Systems& "Yes" / "No" &Did the publication incorporate specific recommender system behavior as a factor for an echo chamber? \\
\hline


\multirow{2}{3cm}
{SOCIAL MEDIA DATA: 
What type of social media data was used?} & Platform(s) & String of Platform analyzed, one variable for each data set that was analyzed in the publication &Which social media platform(s) were analyzed in the publication?\\
\cline{2-4} 

& Data set & String of the data set that was used. Similar data sets were matched. Table \ref{tab:datasets} presents the corpus' data sets.\\
\cline{2-4}
& Countries & String &Which countries came the data from? \\
\cline{2-4}

& Number of Users & One Integer for one data set, not rounded and mean for several data sets on the same platform& How many users were analyzed? \\
\cline{2-4}& Number of Data Points & One Integer for one data set, not rounded and mean for several data sets on the same platform&How many data points were considered (e.g. comments, posts, likes)? \\

\hline
\multirow{2}{3cm}{METHOD: Which methods, operationalization, and metrics are used?} & Method(s) & One of the following: Social Media Data Analysis, Survey, Experiments, Mixed Methods&Which method is used by the authors to research echo chambers? \\
\cline{2-4}

& Metrics and Measures & String(s) of the used metrics and measures (the operationalization) of EC in the paper. See Table \ref{table:echometrics} for metrics and measures in EC research. &Which metrics and measures are utilized in the study's analysis of echo chambers? \\

\hline

\multirow{5}{3cm}{RESULTS ANTECEDENTS: Which mechanisms or antecedents are associated with echo chamber formation?} 

& Political Institutions& "Yes" / "No"  &Does the paper discuss the influence of political institutions in the context of echo chambers creation? \\
\cline{2-4}

& Populism & "Yes" / "No" &Does the publication link its findings to the concept of populism to the creation of echo chamber? \\
\cline{2-4}

& Fragmented Society &  "Yes" / "No" &Does the publication consider a fragmented society as one antecedent of echo chambers?\\ \cline{2-4} 

& Content Moderation and Recommender Systems & "Yes" / "No" &Does the publication explore aspects of content moderation, algorithmic curation, and recommender systems as antecedents or mechanisms for the establishment of echo chambers? \\
\cline{2-4}

& User Behaviour & "Yes" / "No" &Is specific user behavior like cognitive dissonance, selective exposure, or confirmation bias associated with echo chambers?\\
\cline{1-4}

\multirow{5}{3cm}{RESULTS ATTRIBUTES: Which attributes are associated with echo chamber formation?} 

&Active Users & "Yes" / "No" &Does the paper discuss the role of active users in shaping the outcomes related to social media data and echo chambers? \\
\cline{2-4}

& Around Events? &"Yes" / "No"  &Does the publication consider echo chamber creation around specific events? \\
\cline{2-4}

& Mitigation? & "Yes" / "No" &Does the publication address potential mitigation strategies for echo chambers? \\ \cline{2-4} 

& Found EC & "Yes" / "No" &Did the publication find evidence for echo chamber(s)? \\
\cline{2-4} 

& Found No EC & "Yes" / "No"  &Did the publication find evidence against echo chamber(s)? \\

\hline
\multirow{5}{3cm}{RESULTS EFFECTS: Which effects are associated with echo chamber formation?} 

& Toxicity & "Yes" / "No" &Is an increase of toxicity associated with echo chambers? \\
\cline{2-4}

& Emotional Contagion &"Yes" / "No"  &Is an emotional contagion associated with echo chambers? \\
\cline{2-4}

& No Effect & "Yes" / "No"  &Does the publication suggest that there is no significant effect of echo chambers on social media? \\
\cline{2-4}

& Polarization & "Yes" / "No" &Does the publication find evidence for  polarization as an effect in the context of echo chambers? \\ \cline{2-4} 

& Extremism & "Yes" / "No" &Does the publication find evidence for extremism as an effect in the context of echo chambers? \\
\cline{2-4}
& Trust-loss &"Yes" / "No"  &Does the publication find evidence for trust-loss as an effect in the context of echo chambers \\
\cline{2-4}
& Misinformation & "Yes" / "No" &Does the publication find evidence for misinformation as an effect in the context of echo chambers? \\

\hline 

{c|c}
    \end{tabular}
   \caption{Table of the codes from the detailed analysis\label{long}}
\label{tab:detailed_analysis}
\end{table}
\end{small}


==> Tables/table_measures.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lp{8cm}}
\hline
\textbf{Category} & \textbf{Metrics} \\
\hline
\multirow{7}{*}{Ideological Congruence \& Content Alignment} & Ideological congruence \\
& Issue salience \\
& TF-IDF \\
& Content alignment \\
& Cross-cutting content \\
& Campaign affiliation: Frequency of one-sided shared hashtags per user \\
& Activity of users and mentions of parties \\
\hline
\multirow{8}{*}{Polarization \& Homophily} & Political homophily \\
& Fragmentation metric F \\
& Homophily similarity score \\
& Bimodality coefficient \\
& Shares in a given timeframe \\
& Preferences of users and political leaning \\
& User activity per subreddit \\
& Heterogeneity in communities \\
\hline
\multirow{8}{*}{Selective Exposure \& User Preferences} & Selective exposure \\
& Preferences of users \\
& Average nearest-neighbors degree \\
& User leaning \\
& Power distributions \\
& Cross-cutting content \\
& Homogeneous social network intergroup dynamics test \\
& Ideological bias \\
\hline
\multirow{8}{*}{Network Structure \& Centrality} & Assortativity \\
& Linguistic intergroup bias \\
& Modularity \\
& Centrality measures \\
& Flow stability \\
& Socio-demographic features \\
& The cluster's modularity and density \\
& PageRank of nodes within clusters \\
\hline
\multirow{4}{*}{Emotion \& Opinion Dynamics} & Emotion opinion polarization \\
& Information spreading \\
& Political slant \\
& Framing and social conformity \\
\hline

\end{tabular}
\caption{List of CSS Echo Chamber Operationalization Metrics}
\label{table:echometrics}
\end{table}
